Bias Amplification: Large Language Models as Increasingly Biased Media

Model collapse, a phenomenon characterized by performance degradation due to iterative training on synthetic data, has been widely studied. However, its implications for bias amplification, the progressive intensification of pre-existing societal biases in Large Language Models (LLMs), remain significantly underexplored, despite the growing influence of LLMs in shaping online discourse. In this paper, we introduce a open, generational, and long-context benchmark specifically designed to measure political bias amplification in LLMs, leveraging sentence continuation tasks derived from a comprehensive dataset of U.S. political news. Our empirical study using GPT-2 reveals consistent and substantial political bias intensification (e.g., right-leaning amplification) over iterative synthetic training cycles. We evaluate three mitigation strategies, Overfitting, Preservation, and Accumulation, and demonstrate that bias amplification persists independently of model collapse, even when the latter is effectively controlled. Furthermore, we propose a mechanistic analysis approach that identifies neurons correlated with specific phenomena during inference through regression and statistical tests. This analysis uncovers largely distinct neuron populations driving bias amplification and model collapse, underscoring fundamentally different underlying mechanisms. Finally, we supplement our empirical findings with theoretical intuition that explains the separate origins of these phenomena, guiding targeted strategies for bias mitigation.

==> deleted.tex <==
\section{Formal Conditions}
\label{Theoretical Intuition}

In this section, we formalize the conditions for bias amplification, offering an intuitive look at its principal drivers. We then illustrate these ideas using Weighted Maximum Likelihood Estimation (WMLE).

\subsection{The Conditions for Bias Amplification}
\label{Mechanism of Bias Amplification}
The primary factor is referred to as \textbf{bias projection}. It arises when the direction in which the parameters need to move to reduce the loss also coincides with the direction that increases the level of bias on average for a given task. To illustrate this, consider a fine-tuning process in which the pre-trained model parameters $\theta_{t}$ can be expressed as the sum of unbiased and biased components:

    \begin{equation*}
    \theta_{t} = \theta_{t, \text{unbiased}} + \theta_{t, \text{biased}}.
    \end{equation*}
    Specifically, we assume: (1) there exists a unique bias direction, $u$, such that $\theta$ can be decomposed into $\theta_\text{unbiased}$, which is orthogonal to $u$, and $\theta_\text{biased}$, where $|\theta_\text{biased} \cdot u| > 0$; and
(2) the extent of bias in the model is measured by $|\theta_\text{biased} \cdot u|$.
    During gradient-based optimization, the update rule is:
    \begin{equation*}
    \theta_{t+1} = \theta_{t} - \eta \nabla_{\theta} \mathcal{L}_{\text{ft}}(\theta_{t}),
    \end{equation*}
    where $\eta$ is the learning rate, and $\mathcal{L}_{\text{ft}}$ denotes the fine-tuning loss function. Substituting the decomposition of $\theta_{t}$ and taking the projection, we have:
    \begin{equation*}
    \displaystyle \theta_{t+1} = \theta_{t, \text{unbiased}} + \theta_{t, \text{biased}} - \eta \left( \frac{\mathbf{\theta_{t, \text{biased}}}}{\| \mathbf{\theta_{t, \text{biased}}} \|} \right) c_{t}
    \end{equation*}
    where $\displaystyle c_t$ is the \hypertarget{bias projection coefficient}{\emph{bias projection coefficient}}, measuring the projection of the gradient onto the normalized biased component of the parameters:
    \begin{equation}
    c_{t} = \left( \frac{\theta_{t, \text{biased}}}{\| \theta_{t, \text{biased}} \|} \right)^\top \nabla_{\theta} \mathcal{L}_{\text{ft}}(\theta_{t}).
    \end{equation}


    If $\displaystyle c_{t} < 0$, the gradient update will reinforce the biased component, leading to bias amplification, i.e. $\displaystyle \Delta |\theta_{\text{biased}}| > 0$. This occurs because the gradient descent step moves the parameters further in the direction of the existing bias. 

The second is \textbf{sampling error}, akin to statistical approximation error \cite{3.1}. If the model has a pre-existing bias, it inherently assigns higher probabilities to tokens that produce biased outputs. Consequently, during synthetic data generation, unbiased tokens—and thus unbiased samples—are more likely to be lost at each resampling step with a finite sample, though this error vanishes as the sample size approaches infinity. This overrepresents biased patterns in the synthetic data, surpassing the model’s original bias and true next-token probabilities. Sampling error thus complements bias projection by further activating biased neurons in response to the skewed dataset.

By definition, bias projection is a sufficient condition for bias amplification, while sampling error serves as a complementary factor. However, sampling error is a sufficient condition for model collapse to occur with nonzero probability \cite{3.1}. This distinction motivates our investigation into whether bias amplification can occur without model collapse, as this would necessitate additional mitigation strategies beyond those for model collapse.

%The third cause is referred to as \textbf{constraint deficiency}. It occurs when the loss or objective function lacks explicit constraints or regularization to counteract bias projection. As a result, the optimization process does not prevent the reinforcement of bias when bias projection is present. To prevent bias amplification theoretically, the loss function can incorporate de-biasing constraints. Consider a modified fine-tuning objective: $
    %\displaystyle \mathcal{L}_{\text{new}}(\theta) = \mathcal{L}_{\text{original}}(\theta) - \lambda \sum_{i=1}^n \max(0, c^{i}_t)^2 + \gamma \sum_{i=1}^n \min(0, c^{i}_t)^2
    %$, where $c^{i}_t$ represents the \textit{bias projection coefficient} for a specific dimension $i$. $\lambda, \gamma \geq 0 $ are the Lagrangian multipliers for the two constraints. The absence of such constraints allows bias amplification when bias projection is present. 

%Thus, how is the bias amplification related with model collapse? Indeed sampling error has non-zero probability lead to both bias amplification and model collapse but there could be bias projectino even without sampling errors as illustrated in the statistical simulation.


\subsection{Statistical Simulation}
\label{Weighted Maximum Likelihood Estimation}

To simulate a controlled setting without sampling error, we consider a statistical estimation cycle using WMLE\footnote{The mathematical formulation is detailed in Appendix \ref{Mathematical Formulation of WML}.} with a large sample size of each resampling step. Specifically, we generate a pre-training dataset $\mathcal{D}_{\text{pre}}$ with 100,000 samples from a Beta$(3,2)$ distribution, representing a biased pre-training dataset. Using maximum likelihood estimation (MLE), we estimate its probability density function, yielding the pre-trained model $f_{\text{pre}}$.

Next, we fine-tune $f_{\text{pre}}$ to approximate a different distribution, Beta$(2,2)$. We generate 100,000 samples from this distribution, denoted as $D_{\text{real}}$, which serves as the initial fine-tuning dataset. In the first round, we apply weighted maximum likelihood estimation (WMLE) using weights derived from $f_{\text{pre}}$, which encode the pre-existing bias of the pre-trained model. This weighting captures the influence of the pre-trained model's parameters on subsequent training. This produces the fine-tuned model $f_{\text{0}}$. We then generate a synthetic dataset $D_{\text{0}}$ of the same size using $f_{\text{0}}$, initiating the iterative fine-tuning loop. In each subsequent round, WMLE is applied using $D_{\text{k}}$ with weights from $f_{\text{k}}$, resulting in $f_{\text{k+1}}$. This process is repeated iteratively, producing models $f_{\text{1}}$ through $f_{\text{10}}$.





%1. Generate $N$ samples from the estimated distribution of generation $k-1$.

%2. Estimate the parameters using WMLE and the $N$ samples, with weights derived from the estimated pdf of generation $k-1$.
Figure~\ref{fig:WMLE} shows the estimated distributions gradually shift toward the mean of the biased pre-training dataset at \( x=0.6 \), becoming progressively more peaked over generations. This occurs despite further training on samples drawn from Beta$(2,2)$ and synthetic data generated from successive models. The distortion arises because the fine-tuning process disproportionately emphasizes regions where the pre-trained distribution assigns higher probability, leading to biased learning. For comparison, Figure~\ref{fig:MLE} presents the results using standard MLE without weighting. In this case, the estimated distributions remain stable across generations, accurately representing the Beta$(2,2)$ distribution.
